Comparing the Effects of DNS, DoT, and DoH on Web Performance

Nearly every service on the Internet relies on the Domain Name System (DNS), which translates a human-readable name to an IP address before two endpoints can communicate. Today, DNS traffic is unencrypted, leaving users vulnerable to eavesdropping and tampering. Past work has demonstrated that DNS queries can reveal a user's browsing history and even what smart devices they are using at home. In response to these privacy concerns, two new protocols have been proposed: DNS-over-HTTPS (DoH) and DNS-over-TLS (DoT). Instead of sending DNS queries and responses in the clear, DoH and DoT establish encrypted connections between users and resolvers. By doing so, these protocols provide privacy and security guarantees that traditional DNS (Do53) lacks. In this paper, we measure the effect of Do53, DoT, and DoH on query response times and page load times from five global vantage points. We find that although DoH and DoT response times are generally higher than Do53, both protocols can perform better than Do53 in terms of page load times. However, as throughput decreases and substantial packet loss and latency are introduced, web pages load fastest with Do53. Additionally, web pages successfully load more often with Do53 and DoT than DoH. Based on these results, we provide several recommendations to improve DNS performance, such as opportunistic partial responses and wire format caching.

==> sections/setup.tex <==
\section{Setup}\label{sec:setup}

To ensure that our results for page load time and DNS resolution are generalizable, we perform measurements across various website lists, resolvers and networks.
This allows us to not only measure simulate browser experience for different users, but also understand how DNS, DoH, and DoT perform under poor network conditions.
We describe our choices of websites, resolvers, and networks below.

\subsection{Websites}

We measured the top 1k websites on the Tranco top-list to understand browser performance for the average user~\cite{le2019tranco}. Furthermore, we measured the bottom 1k of the top 100k websites to understand browser performance for websites are less commonly visited. 
We chose to measure the tail of the top 100k instead of the tail of the top 1m because many websites in the latter are no longer available. 
Furthermore, there is significant churn in the tail of top 1m, which means that we would not be accurately measuring browser performance for the tail across our experiment.

\subsection{Resolvers}

We also want to measure the relationship between recursive resolver choice, DNS transport, and browser performance.
We chose three popular recursive resolvers: Google, Quad9, and Cloudflare.
Each resolvers offers public resolution for DNS, DoT, and DoH.

DNS and DoH are natively supported in Firefox.
However, as of April 2019, DoT must be configured by using a stub resolver on a user's machine out side of Firefox.
For our experiment, we used Stubby for DoT resolution, a stub resolver based on getdns.
Stubby works by listening for DNS requests on on a loopback address. 
All DNS requests received by Stubby would then be send out to a recursive resolver over DoT.
We modified /etc/resolv.conf on a Debian system to point to the loopback address used by Stubby.
This would force all DNS requests initiated by Firefox to be sent over DoT.

We also used the local resolver for Princeton University to measure page load times and DNS performance. 
However, this resolver only supports DNS, and not DoT or DoH. Thus, this resolver serves as a baseline for browser performance over DNS on a campus network.

\subsection{Networks}\label{sec:networks}

We also wanted to understand the relationship between browser performance, DNS transports, and choice of networks.
To do so, we performed our measurements across three different networks.

The first network we chose for our measurement is the Princeton University campus network.
It is a well-connected network to Cloudflare, Quad9, and Google. 
We chose this network to measure the best case effect of different DNS transports on web performance.

The second network we chose for our measurement is Comcast Business.
It is a fairly well-connected network to Cloudflare and Google, but not to Quad9. 
We chose this network to measure the effect average case effect of different DNS transports on web performance for commercial ISP subscribers.

The third network we chose for our measurement is Comcast Business, but with traffic shaping applied to simulate mobile device performance.
We shaped outgoing traffic with an increased latency of 53.3m and a jitter of 1ms.
We also dropped 0.5\% of packets.
Finally, we shaped our uplink rate to 7.44Mb/s and our downlink rate to 22.1Mb/s.
These settings are based on an OpenSignal report of mobile network experience across providers~\cite{opensignal}.

We believe it is important to simulate 4G performance because an increasing number of users are browsing the web through their phones, and organizations like Cloudflare have released apps for sending mobile traffic over encrypted DNS transports.


==> tables/failure.tex <==
\begin{table*}[t!]
  \centering
  \footnotesize
  \rowcolors{1}{}{lightgray}
  \renewcommand{\arraystretch}{1.1}
  \begin{tabularx}{\textwidth}{Xlrrrrrrrrrr}
    & & \textbf{Default} & \multicolumn{3}{c}{\textbf{Quad9}} & \multicolumn{3}{c}{\textbf{Google}} & \multicolumn{3}{c}{\textbf{Cloudflare}}\\
    \rowcolor{black}\cline{3-12}
    \rowcolor{white}\textbf{Connectivity} & \textbf{Status} & Do53 & Do53 & DoT & DoH & Do53 & DoT & DoH & Do53 & DoT & DoH\\
    \arrayrulecolor{black}\hline
      \cellcolor{white}
        & Successful
        & 76.11\%
        & 76.29\%
        & 75.53\%
        & 73.65\%
        & 76.08\%
        & 75.51\%
        & 74.63\%
        & 76.39\%
        & 76.24\%
        & 75.13\%
        \\
      \cellcolor{white}
        & Page-load Timeout
        & 9.77\%
        & 9.61\%
        & 10.05\%
        & 9.18\%
        & 9.95\%
        & 9.83\%
        & 9.63\%
        & 9.71\%
        & 9.70\%
        & 9.47\%
        \\
      \cellcolor{white}
        & DNS Error
        & 9.44\%
        & 9.46\%
        & 9.43\%
        & 10.57\%
        & 9.29\%
        & 9.28\%
        & 9.72\%
        & 9.32\%
        & 9.27\%
        & 9.42\%
        \\
      \cellcolor{white}
        & Selenium Error
        & 1.84\%
        & 1.83\%
        & 1.89\%
        & 1.74\%
        & 1.86\%
        & 1.89\%
        & 1.86\%
        & 1.86\%
        & 1.86\%
        & 1.79\%
        \\
      \cellcolor{white}\multirow{-5}{*}{Default network}
        & Other Error
        & 4.68\%
        & 4.64\%
        & 4.99\%
        & 6.60\%
        & 4.68\%
        & 5.38\%
        & 6.02\%
        & 4.58\%
        & 4.79\%
        & 5.98\%
        \\
    \arrayrulecolor{gray}\hline
    \cellcolor{lightgray}
        & Successful
        & 76.59\%
        & 76.92\%
        & 76.32\%
        & 75.08\%
        & 76.91\%
        & 77.43\%
        & 76.55\%
        & 77.18\%
        & 77.58\%
        & 77.48\%
        \\
      \cellcolor{lightgray}
        & Page-load Timeout
        & 10.49\%
        & 10.53\%
        & 11.23\%
        & 10.14\%
        & 10.47\%
        & 10.55\%
        & 10.44\%
        & 10.59\%
        & 10.33\%
        & 10.23\%
        \\
      \cellcolor{lightgray}
        & DNS Error
        & 9.37\%
        & 9.46\%
        & 9.47\%
        & 11.63\%
        & 9.27\%
        & 9.28\%
        & 10.09\%
        & 9.30\%
        & 9.29\%
        & 9.51\%
        \\
      \cellcolor{lightgray}
        & Selenium Error
        & 1.86\%
        & 1.88\%
        & 1.85\%
        & 1.79\%
        & 1.80\%
        & 1.72\%
        & 1.82\%
        & 1.74\%
        & 1.86\%
        & 1.84\%
        \\
      \cellcolor{lightgray}\multirow{-5}{*}{4G network}
        & Other Error
        & 3.55\%
        & 3.09\%
        & 2.98\%
        & 3.15\%
        & 3.35\%
        & 2.74\%
        & 2.92\%
        & 2.93\%
        & 2.80\%
        & 2.78\%
        \\
    \arrayrulecolor{gray}\hline
    \cellcolor{white}
        & Successful
        & 77.42\%
        & 77.10\%
        & 76.65\%
        & 75.18\%
        & 77.18\%
        & 77.59\%
        & 76.24\%
        & 76.97\%
        & 77.92\%
        & 77.89\%
        \\
      \cellcolor{white}
        & Page-load Timeout
        & 10.42\%
        & 10.74\%
        & 11.19\%
        & 9.46\%
        & 10.65\%
        & 10.48\%
        & 10.40\%
        & 10.52\%
        & 10.23\%
        & 9.98\%
        \\
      \cellcolor{white}
        & DNS Error
        & 9.36\%
        & 9.39\%
        & 9.42\%
        & 12.16\%
        & 9.23\%
        & 9.23\%
        & 10.47\%
        & 9.29\%
        & 9.25\%
        & 9.50\%
        \\
      \cellcolor{white}
        & Selenium Error
        & 1.81\%
        & 1.60\%
        & 1.71\%
        & 1.89\%
        & 1.71\%
        & 1.76\%
        & 1.87\%
        & 1.71\%
        & 1.72\%
        & 1.69\%
        \\
      \cellcolor{white}\multirow{-5}{*}{Lossy 4G network}
        & Other Error
        & 2.80\%
        & 2.77\%
        & 2.74\%
        & 3.20\%
        & 2.94\%
        & 2.70\%
        & 2.89\%
        & 3.22\%
        & 2.60\%
        & 2.63\%
        \\
    \arrayrulecolor{gray}\hline
    \cellcolor{lightgray}
        & Successful
        & 22.65\%
        & 22.29\%
        & 22.13\%
        & 9.86\%
        & 22.45\%
        & 22.67\%
        & 13.66\%
        & 22.46\%
        & 22.42\%
        & 17.62\%
        \\
      \cellcolor{lightgray}
        & Page-load Timeout
        & 66.21\%
        & 66.50\%
        & 66.54\%
        & 29.02\%
        & 66.46\%
        & 66.02\%
        & 40.63\%
        & 66.40\%
        & 66.51\%
        & 51.40\%
        \\
      \cellcolor{lightgray}
        & DNS Error
        & 9.32\%
        & 9.39\%
        & 9.50\%
        & 60.11\%
        & 9.23\%
        & 9.32\%
        & 44.39\%
        & 9.25\%
        & 9.25\%
        & 29.48\%
        \\
      \cellcolor{lightgray}
        & Selenium Error
        & 1.48\%
        & 1.53\%
        & 1.56\%
        & 0.65\%
        & 1.55\%
        & 1.70\%
        & 0.95\%
        & 1.59\%
        & 1.51\%
        & 1.22\%
        \\
      \cellcolor{lightgray}\multirow{-5}{*}{3G network}
        & Other Error
        & 1.82\%
        & 1.82\%
        & 1.83\%
        & 1.01\%
        & 1.86\%
        & 1.99\%
        & 1.32\%
        & 1.89\%
        & 1.82\%
        & 1.50\%
        \\
    \arrayrulecolor{black}\hline
  \end{tabularx}
  \caption{Successful website page-loads and error percentages for different network conditions.}
  \label{tab:failure}
\end{table*}


==> tables/failure_3g.tex <==
\begin{table*}[h]
  \centering
  \footnotesize
  \rowcolors{1}{}{lightgray}
  \renewcommand{\arraystretch}{1.2}
  \begin{tabularx}{\textwidth}{Xlrrrrrrrrrr}
    & & \textbf{Default} & \multicolumn{3}{c}{\textbf{Quad9}} & \multicolumn{3}{c}{\textbf{Google}} & \multicolumn{3}{c}{\textbf{Cloudflare}}\\
    \rowcolor{black}\cline{3-12}
    \rowcolor{white}\textbf{Connectivity} & \textbf{Status} & Do53 & Do53 & DoT & DoH & Do53 & DoT & DoH & Do53 & DoT & DoH\\
    \arrayrulecolor{gray}\hline
    \cellcolor{lightgray}
        & Successful
        & 28.14\%
        & 27.79\%
        & 27.48\%
        & 0.28\%
        & 28.34\%
        & 28.21\%
        & 0.46\%
        & 28.10\%
        & 27.87\%
        & 20.06\%
        \\
      \cellcolor{lightgray}
        & Page-load Timeout
        & 60.12\%
        & 60.32\%
        & 60.68\%
        & 0.47\%
        & 59.82\%
        & 59.97\%
        & 0.71\%
        & 60.02\%
        & 60.31\%
        & 41.32\%
        \\
      \cellcolor{lightgray}
        & DNS Error
        & 9.73\%
        & 9.80\%
        & 9.82\%
        & 99.24\%
        & 9.77\%
        & 9.76\%
        & 98.80\%
        & 9.83\%
        & 9.76\%
        & 37.15\%
        \\
      \cellcolor{lightgray}
        & Selenium Error
        & 1.54\%
        & 1.59\%
        & 1.58\%
        & 0.02\%
        & 1.70\%
        & 1.59\%
        & 0.01\%
        & 1.65\%
        & 1.54\%
        & 1.07\%
        \\
      \cellcolor{lightgray}\multirow{-5}{*}{Cellular 3G}
        & Other Error
        & 2.01\%
        & 2.08\%
        & 2.02\%
        & 0.02\%
        & 2.07\%
        & 2.06\%
        & 0.03\%
        & 2.06\%
        & 2.06\%
        & 1.47\%
        \\
    \arrayrulecolor{black}\hline
  \end{tabularx}
  \caption{Successful website page-loads and error percentages for different network conditions.}
  \label{tab:failure}
\end{table*}

==> tables/failure_4g.tex <==
\begin{table*}[h]
  \centering
  \footnotesize
  \rowcolors{1}{}{lightgray}
  \renewcommand{\arraystretch}{1.2}
  \begin{tabularx}{\textwidth}{Xlrrrrrrrrrr}
    & & \textbf{Default} & \multicolumn{3}{c}{\textbf{Quad9}} & \multicolumn{3}{c}{\textbf{Google}} & \multicolumn{3}{c}{\textbf{Cloudflare}}\\
    \rowcolor{black}\cline{3-12}
    \rowcolor{white}\textbf{Connectivity} & \textbf{Status} & Do53 & Do53 & DoT & DoH & Do53 & DoT & DoH & Do53 & DoT & DoH\\
    \arrayrulecolor{gray}\hline
    \cellcolor{lightgray}
        & Successful
        & 80.14\%
        & 80.16\%
        & 79.05\%
        & 73.23\%
        & 80.07\%
        & 79.76\%
        & 0.04\%
        & 80.02\%
        & 79.71\%
        & 78.61\%
        \\
      \cellcolor{lightgray}
        & Page-load Timeout
        & 7.60\%
        & 7.64\%
        & 8.27\%
        & 6.70\%
        & 7.82\%
        & 7.71\%
        & 0.02\%
        & 7.86\%
        & 7.75\%
        & 7.22\%
        \\
      \cellcolor{lightgray}
        & DNS Error
        & 9.05\%
        & 9.08\%
        & 9.08\%
        & 15.95\%
        & 8.97\%
        & 9.03\%
        & 99.93\%
        & 9.02\%
        & 9.00\%
        & 9.77\%
        \\
      \cellcolor{lightgray}
        & Selenium Error
        & 1.79\%
        & 1.69\%
        & 1.79\%
        & 1.72\%
        & 1.71\%
        & 1.79\%
        & 0.00\%
        & 1.84\%
        & 1.67\%
        & 1.86\%
        \\
      \cellcolor{lightgray}\multirow{-5}{*}{Cellular 4G}
        & Other Error
        & 3.21\%
        & 3.12\%
        & 3.60\%
        & 4.12\%
        & 3.13\%
        & 3.49\%
        & 0.01\%
        & 3.10\%
        & 3.54\%
        & 4.39\%
        \\
    \arrayrulecolor{black}\hline
  \end{tabularx}
  \caption{Successful website page-loads and error percentages for different network conditions.}
  \label{tab:failure}
\end{table*}

==> tables/failure_4g_lossy.tex <==
\begin{table*}[h]
  \centering
  \footnotesize
  \rowcolors{1}{}{lightgray}
  \renewcommand{\arraystretch}{1.2}
  \begin{tabularx}{\textwidth}{Xlrrrrrrrrrr}
    & & \textbf{Default} & \multicolumn{3}{c}{\textbf{Quad9}} & \multicolumn{3}{c}{\textbf{Google}} & \multicolumn{3}{c}{\textbf{Cloudflare}}\\
    \rowcolor{black}\cline{3-12}
    \rowcolor{white}\textbf{Connectivity} & \textbf{Status} & Do53 & Do53 & DoT & DoH & Do53 & DoT & DoH & Do53 & DoT & DoH\\
    \arrayrulecolor{gray}\hline
    \cellcolor{white}
        & Successful
        & 78.31\%
        & 78.20\%
        & 77.89\%
        & 65.29\%
        & 78.23\%
        & 78.16\%
        & 0.20\%
        & 78.29\%
        & 78.13\%
        & 76.95\%
        \\
      \cellcolor{white}
        & Page-load Timeout
        & 8.25\%
        & 8.32\%
        & 8.67\%
        & 6.70\%
        & 8.32\%
        & 8.19\%
        & 0.00\%
        & 8.24\%
        & 8.16\%
        & 8.01\%
        \\
      \cellcolor{white}
        & DNS Error
        & 9.93\%
        & 9.95\%
        & 9.97\%
        & 24.27\%
        & 9.91\%
        & 9.94\%
        & 99.80\%
        & 9.95\%
        & 9.95\%
        & 10.76\%
        \\
      \cellcolor{white}
        & Selenium Error
        & 1.97\%
        & 1.98\%
        & 1.95\%
        & 1.72\%
        & 1.96\%
        & 2.01\%
        & 0.00\%
        & 1.99\%
        & 1.96\%
        & 2.01\%
        \\
      \cellcolor{white}\multirow{-5}{*}{Cellular 4G Lossy}
        & Other Error
        & 3.51\%
        & 3.53\%
        & 3.47\%
        & 3.75\%
        & 3.54\%
        & 3.70\%
        & 0.00\%
        & 3.53\%
        & 3.76\%
        & 4.28\%
        \\
    \arrayrulecolor{black}\hline
  \end{tabularx}
  \caption{Successful website page-loads and error percentages for different network conditions.}
  \label{tab:failure}
\end{table*}

==> tables/failure_default.tex <==
\begin{table*}[h]
  \centering
  \footnotesize
  \rowcolors{1}{}{lightgray}
  \renewcommand{\arraystretch}{1.2}
  \begin{tabularx}{\textwidth}{Xlrrrrrrrrrr}
    & & \textbf{Default} & \multicolumn{3}{c}{\textbf{Quad9}} & \multicolumn{3}{c}{\textbf{Google}} & \multicolumn{3}{c}{\textbf{Cloudflare}}\\
    \rowcolor{black}\cline{3-12}
    \rowcolor{white}\textbf{Connectivity} & \textbf{Status} & Do53 & Do53 & DoT & DoH & Do53 & DoT & DoH & Do53 & DoT & DoH\\
    \arrayrulecolor{black}\hline
      \cellcolor{white}
        & Successful
        & 78.67\%
        & 78.54\%
        & 78.46\%
        & 76.67\%
        & 78.49\%
        & 78.63\%
        & 3.39\%
        & 78.70\%
        & 78.65\%
        & 78.85\%
        \\
      \cellcolor{white}
        & Page-load Timeout
        & 7.46\%
        & 7.37\%
        & 7.70\%
        & 6.79\%
        & 7.25\%
        & 7.33\%
        & 0.24\%
        & 7.48\%
        & 7.47\%
        & 7.21\%
        \\
      \cellcolor{white}
        & DNS Error
        & 9.47\%
        & 9.54\%
        & 9.64\%
        & 12.47\%
        & 9.50\%
        & 9.51\%
        & 96.27\%
        & 9.51\%
        & 9.46\%
        & 9.90\%
        \\
      \cellcolor{white}
        & Selenium Error
        & 1.79\%
        & 1.75\%
        & 1.73\%
        & 1.74\%
        & 1.79\%
        & 1.72\%
        & 0.08\%
        & 1.69\%
        & 1.74\%
        & 1.78\%
        \\
      \cellcolor{white}\multirow{-5}{*}{Wired University}
        & Other Error
        & 4.40\%
        & 4.56\%
        & 4.21\%
        & 4.07\%
        & 4.76\%
        & 4.53\%
        & 0.10\%
        & 4.31\%
        & 4.41\%
        & 4.04\%
        \\
    \arrayrulecolor{black}\hline
  \end{tabularx}
  \caption{Successful website page-loads and error percentages for different network conditions.}
  \label{tab:failure}
\end{table*}

==> tables/failure_seoul_3g_cf.tex <==
\begin{table*}[h]
  \centering
  \footnotesize
  \rowcolors{1}{}{lightgray}
  \renewcommand{\arraystretch}{1.2}
  \begin{tabularx}{\textwidth}{Xlrrrrrrrrrr}
    & & \textbf{Default} & \multicolumn{3}{c}{\textbf{Quad9}} & \multicolumn{3}{c}{\textbf{Google}} & \multicolumn{3}{c}{\textbf{Cloudflare}}\\
    \rowcolor{black}\cline{3-12}
    \rowcolor{white}\textbf{Connectivity} & \textbf{Status} & Do53 & Do53 & DoT & DoH & Do53 & DoT & DoH & Do53 & DoT & DoH\\
    \arrayrulecolor{gray}\hline
    \cellcolor{lightgray}
        & Successful
        & 25.56\%
        & 25.40\%
        & 17.91\%
        \\
      \cellcolor{lightgray}
        & Page-load Timeout
        & 62.75\%
        & 62.97\%
        & 42.24\%
        \\
      \cellcolor{lightgray}
        & DNS Error
        & 9.62\%
        & 9.59\%
        & 38.40\%
        \\
      \cellcolor{lightgray}
        & Selenium Error
        & 1.61\%
        & 1.60\%
        & 1.10\%
        \\
      \cellcolor{lightgray}\multirow{-5}{*}{Cellular 3G}
        & Other Error
        & 2.07\%
        & 2.03\%
        & 1.46\%
        \\
    \arrayrulecolor{black}\hline
  \end{tabularx}
  \caption{Successful website page-loads and error percentages for different network conditions.}
  \label{tab:failure}
\end{table*}

==> tables/failure_seoul_4g_cf.tex <==
\begin{table*}[h]
  \centering
  \footnotesize
  \rowcolors{1}{}{lightgray}
  \renewcommand{\arraystretch}{1.2}
  \begin{tabularx}{\textwidth}{Xlrrrrrrrrrr}
    & & \textbf{Default} & \multicolumn{3}{c}{\textbf{Quad9}} & \multicolumn{3}{c}{\textbf{Google}} & \multicolumn{3}{c}{\textbf{Cloudflare}}\\
    \rowcolor{black}\cline{3-12}
    \rowcolor{white}\textbf{Connectivity} & \textbf{Status} & Do53 & Do53 & DoT & DoH & Do53 & DoT & DoH & Do53 & DoT & DoH\\
    \arrayrulecolor{gray}\hline
    \cellcolor{lightgray}
        & Successful
        & 77.34\%
        & 77.28\%
        & 66.34\%
        \\
      \cellcolor{lightgray}
        & Page-load Timeout
        & 9.86\%
        & 9.91\%
        & 8.10\%
        \\
      \cellcolor{lightgray}
        & DNS Error
        & 9.53\%
        & 9.53\%
        & 22.85\%
        \\
      \cellcolor{lightgray}
        & Selenium Error
        & 1.90\%
        & 1.88\%
        & 1.66\%
        \\
      \cellcolor{lightgray}\multirow{-5}{*}{Cellular 4G}
        & Other Error
        & 3.27\%
        & 3.28\%
        & 2.71\%
        \\
    \arrayrulecolor{black}\hline
  \end{tabularx}
  \caption{Successful website page-loads and error percentages for different network conditions.}
  \label{tab:failure}
\end{table*}


==> tables/failure_seoul_4g_lossy_cf.tex <==
\begin{table*}[h]
  \centering
  \footnotesize
  \rowcolors{1}{}{lightgray}
  \renewcommand{\arraystretch}{1.2}
  \begin{tabularx}{\textwidth}{Xlrrrrrrrrrr}
    & & \textbf{Default} & \multicolumn{3}{c}{\textbf{Quad9}} & \multicolumn{3}{c}{\textbf{Google}} & \multicolumn{3}{c}{\textbf{Cloudflare}}\\
    \rowcolor{black}\cline{3-12}
    \rowcolor{white}\textbf{Connectivity} & \textbf{Status} & Do53 & Do53 & DoT & DoH & Do53 & DoT & DoH & Do53 & DoT & DoH\\
    \arrayrulecolor{gray}\hline
    \cellcolor{white}
        & Successful
        & 76.97\%
        & 77.40\%
        & 66.52\%
        \\
      \cellcolor{white}
        & Page-load Timeout
        & 10.11\%
        & 9.86\%
        & 8.18\%
        \\
      \cellcolor{white}
        & DNS Error
        & 9.62\%
        & 9.61\%
        & 22.70\%
        \\
      \cellcolor{white}
        & Selenium Error
        & 1.98\%
        & 1.85\%
        & 1.62\%
        \\
      \cellcolor{white}\multirow{-5}{*}{Cellular 4G Lossy}
        & Other Error
        & 3.30\%
        & 3.13\%
        & 2.60\%
        \\
    \arrayrulecolor{black}\hline
  \end{tabularx}
  \caption{Successful website page-loads and error percentages for different network conditions.}
  \label{tab:failure}
\end{table*}


==> tables/failure_seoul_default_cf.tex <==
\begin{table*}[h]
  \centering
  \footnotesize
  \rowcolors{1}{}{lightgray}
  \renewcommand{\arraystretch}{1.2}
  \begin{tabularx}{\textwidth}{Xlrrrrrrrrrr}
    & & \textbf{Default} & \multicolumn{3}{c}{\textbf{Quad9}} & \multicolumn{3}{c}{\textbf{Google}} & \multicolumn{3}{c}{\textbf{Cloudflare}}\\
    \rowcolor{black}\cline{3-12}
    \rowcolor{white}\textbf{Connectivity} & \textbf{Status} & Do53 & Do53 & DoT & DoH & Do53 & DoT & DoH & Do53 & DoT & DoH\\
    \arrayrulecolor{black}\hline
      \cellcolor{white}
        & Successful
        & 78.34\%
        & 78.04\%
        & 78.19\%
        \\
      \cellcolor{white}
        & Page-load Timeout
        & 8.96\%
        & 9.01\%
        & 8.58\%
        \\
      \cellcolor{white}
        & DNS Error
        & 9.30\%
        & 9.29\%
        & 9.84\%
        \\
      \cellcolor{white}
        & Selenium Error
        & 1.83\%
        & 1.94\%
        & 1.87\%
        \\
      \cellcolor{white}\multirow{-5}{*}{Wired University}
        & Other Error
        & 3.40\%
        & 3.66\%
        & 3.39\%
        \\
    \arrayrulecolor{black}\hline
  \end{tabularx}
  \caption{Successful website page-loads and error percentages for different network conditions.}
  \label{tab:failure}
\end{table*}

==> tables/latency.tex <==
\begin{table*}[h]
  \centering
  \footnotesize
  \rowcolors{1}{}{lightgray}
  \renewcommand{\arraystretch}{1.2}
  \begin{tabularx}{\textwidth}{Xlrrrrr}
    \rowcolor{white}
      \textbf{Connectivity}
      & \textbf{Recursor}
      & \textbf{Minimum Latency}
      & \textbf{Average Latency}
      & \textbf{Maximum Latency}
      & \textbf{Standard Deviation \textsigma}
      & \textbf{Observations}
      \\
    \arrayrulecolor{black}\hline
      \cellcolor{white}
        & Default
        & 0.28ms
        & 0.44ms
        & 11.42ms
        & 0.11ms
        & 49,999
        \\
      \cellcolor{white}
        & Quad9
        & 2.20ms
        & 3.00ms
        & 55.29ms
        & 0.34ms
        & 149,993
        \\
      \cellcolor{white}
        & Google
        & 2.54ms
        & 2.94ms
        & 53.18ms
        & 0.34ms
        & 149,987
        \\
      \cellcolor{white}
        \cellcolor{white}\multirow{-4}{*}{Wired University}
        & Cloudflare
        & 2.36ms
        & 2.85ms
        & 166.06ms
        & 0.62ms
        & 149,964
        \\
    \arrayrulecolor{gray}\hline
      \cellcolor{lightgray}
        & Default
        & 52.67ms
        & 53.91ms
        & 90.93ms
        & 0.71ms
        & 49,744
        \\
      \cellcolor{lightgray}
        & Quad9
        & 54.68ms
        & 56.46ms
        & 291.57ms
        & 1.26ms
        & 149,240
        \\
      \cellcolor{lightgray}
        & Google
        & 54.91ms
        & 56.39ms
        & 215.91ms
        & 1.07ms
        & 149,172
        \\
      \cellcolor{lightgray}\multirow{-4}{*}{Cellular 4G}
        & Cloudflare
        & 54.77ms
        & 56.29ms
        & 263.51ms
        & 1.10ms
        & 149,204
        \\
    \arrayrulecolor{gray}\hline
      \cellcolor{white}
        & Default
        & 52.67ms
        & 53.93ms
        & 92.11ms
        & 0.68ms
        & 49,244
        \\
      \cellcolor{white}
        & Quad9
        & 54.68ms
        & 56.85ms
        & 336.34ms
        & 9.73ms
        & 147,489
        \\
      \cellcolor{white}
        & Google
        & 54.95ms
        & 56.57ms
        & 333.59ms
        & 6.48ms
        & 147,659
        \\
      \cellcolor{white}
        \cellcolor{white}\multirow{-4}{*}{Cellular 4G Lossy}
        & Cloudflare
        & 54.72ms
        & 56.55ms
        & 335.53ms
        & 8.55ms
        & 147,565
        \\
    \arrayrulecolor{gray}\hline
      \cellcolor{lightgray}
        & Default
        & 142.44ms
        & 150.75ms
        & 449.63ms
        & 5.14ms
        & 48,937
        \\
      \cellcolor{lightgray}
        & Quad9
        & 144.54ms
        & 153.64ms
        & 622.37ms
        & 10.80ms
        & 146,466
        \\
      \cellcolor{lightgray}
        & Google
        & 144.78ms
        & 153.38ms
        & 456.77ms
        & 8.00ms
        & 146,652
        \\
      \cellcolor{lightgray}\multirow{-4}{*}{Cellular 3G}
        & Cloudflare
        & 144.57ms
        & 153.41ms
        & 454.11ms
        & 10.30ms
        & 146,660
        \\
    \arrayrulecolor{black}\hline
  \end{tabularx}
  \caption{Recursor latency characteristics for different network conditions from Frankfurt.}
  \label{tab:latency}
\end{table*}


==> tables/latency_frankfurt_default.tex <==
\begin{table*}[h]
  \centering
  \footnotesize
  \rowcolors{1}{}{lightgray}
  \renewcommand{\arraystretch}{1.2}
  \begin{tabularx}{\textwidth}{Xlrrrrr}
    \rowcolor{white}
      \textbf{Connectivity}
      & \textbf{Recursor}
      & \textbf{Minimum Latency}
      & \textbf{Average Latency}
      & \textbf{Maximum Latency}
      & \textbf{Standard Deviation \textsigma}
      & \textbf{Observations}
      \\
    \arrayrulecolor{black}\hline
      \cellcolor{white}
        & Quad9
        & 0.97ms
        & 1.42ms
        & 22.62ms
        & 0.27ms
        & 165,440
        \\
      \cellcolor{white}
        & Google
        & 0.47ms
        & 1.00ms
        & 8.18ms
        & 0.21ms
        & 165,479
        \\
      \cellcolor{white}
        \cellcolor{white}\multirow{-4}{*}{Wired University}
        & Cloudflare
        & 0.43ms
        & 1.03ms
        & 6805.60ms
        & 18.10ms
        & 165,397
        \\
    \arrayrulecolor{black}\hline
  \end{tabularx}
  \caption{Recursor latency characteristics for different network conditions.}
  \label{tab:latency}
\end{table*}

==> tables/latency_seoul_default.tex <==
\begin{table*}[h]
  \centering
  \footnotesize
  \rowcolors{1}{}{lightgray}
  \renewcommand{\arraystretch}{1.2}
  \begin{tabularx}{\textwidth}{Xlrrrrr}
    \rowcolor{white}
      \textbf{Connectivity}
      & \textbf{Recursor}
      & \textbf{Minimum Latency}
      & \textbf{Average Latency}
      & \textbf{Maximum Latency}
      & \textbf{Standard Deviation \textsigma}
      & \textbf{Observations}
      \\
    \arrayrulecolor{black}\hline
      \cellcolor{white}
        & Quad9
        & 1.06ms
        & 1.95ms
        & 307.02ms
        & 6.02ms
        & 254,737
        \\
      \cellcolor{white}
        & Google
        & 30.01ms
        & 30.22ms
        & 47.25ms
        & 0.53ms
        & 261,190
        \\
      \cellcolor{white}
        \cellcolor{white}\multirow{-4}{*}{Wired University}
        & Cloudflare
        & 26.46ms
        & 26.65ms
        & 38.12ms
        & 0.44ms
        & 261,184
        \\
    \arrayrulecolor{black}\hline
  \end{tabularx}
  \caption{Recursor latency characteristics for different network conditions.}
  \label{tab:latency}
\end{table*}
